Complete Angular Distributions of the Deuteron Photo-Disintegration Reaction in the Few GeV Region

The study of two body deuteron photo-disintegration is ideal for investigating the transition region from meson exchange to the Quantum Chromo Dynamics (QCD) regime because of its simplicity and amenability to calculation. In the past years, the theoretical efforts have been focused in two different directions: extending at higher energies the models based on meson exchange, and improving the models inspired by QCD principles to extrapolate their predictions at lower energies, in order to find out the approach that best describes the experimental data and in which energy region the transition between the two descriptions takes place.

==> prima.tex <==
\renewcommand{\baselinestretch}{1.0}
\pagestyle{empty}
\bigskip
\vspace{6cm}
\begin{center}
\renewcommand{\baselinestretch}{1.5}
.

\Large
{Dottorato di Ricerca in Fisica\\ 
(XV ciclo)\\}
\vspace{1cm}

\begin{figure}[ht]
\begin{center}
\leavevmode
\epsfig{file=scan/roma3.eps,width=2cm}
\end{center}
\end{figure}

{Universit\`a degli Studi Roma Tre\\}
%\large {INFN, Laboratori Nazionali di Frascati\\
%Jefferson Lab\\}

\vspace{2cm}

\LARGE{\mbox{\bf Complete Angular Distributions of the}\\ \mbox{\bf $\gamma d \rightarrow pn$ Reaction in the Few GeV Region} }
{\Large \\by\\ {\em Federico Ronchetti}
}
\vspace{2cm}

{\Large Thesis Submitted in Fulfillment of the \\Requirements for the Degree \\ {\em Doctor of Philosophy}}

\end{center}


==> ringra.tex <==
\newpage
\addcontentsline{toc}{chapter}{Aknowledgments}
\renewcommand{\baselinestretch}{1.0}
\thispagestyle{empty}
\markboth{}{}
\begin{center}
\section*{Aknowledgments}
\end{center}

\indent
\par

I want to thank Enzo for giving me the opportunity 
to work in his research group and for his continuous attention 
in improving my work and my (and everybody's) 
way of thinking and reasoning.\\

Then, I want to thank Patrizia for her effort 
in coordinating this analysis project since 1999 
and for her personal friendship.\\

Many thanks I owe to Marco, for showing me the skills needed
by the good experimentalist. I am sure I have not learned them
all, nevertheless I shall have the opportunity to recover.\\

Collective thanks go to the whole Frascati Group. 
I consider all of them friends much more than colleagues. \\

I do not forget Leonid and Vera, for giving the 
theoretical support to this work 
and for reviewing it with me. 
I wish we had more time to discuss so 
I could pose them always the same questions.\\

A special thank goes to those who gave me a hand, 
or both hands, in dealing with this monkey thing called \LaTeX{}. \\

Finally, I want to thank my parents and wife Anna Paola.\\
\begin{flushright}
Federico~~~~~~~~~~~~~~~~~~~~~
\end{flushright}
			










==> scan/g2_data_proc/eff/analisi.tex <==

\pagenumbering{arabic}	          
\chapter{Data Reduction and Analysis}
%\pagenumbering{arabic}
%==========================================================================
\section{Introduction}
\indent
\par


\section{Overview of the CLAS offline software}
\indent
\par


\section{Photon flux normalization}
\indent
\par


\section{CLAS detector efficiency}
\indent
\par

About 80\% of the triggers collected during the data taking were of the type $\gamma d \rightarrow A X$, 
where $A$ is a positively charged particle with quantum numbers compatible with the inital state
considered.
This charged trigger was chosen lousy enough since the beam time assigned for the data taking 
was shared among several proposals [ref g2 proposals]. In addition, a second neutral trigger 
was used for the remaining 20\% of the data acquisition rate.

In the case of deuteron two body break up we are intersted only by a subset of the above triggers, 
containing just one single proton in the final state.
The photodisintegration event is then identified looking at the missing mass of the neutron.

The extraction of the final cross section information needs the evaluation of several quantities, 
according to the relation

\begin{equation}
\label{expcrosssect}
\frac{d\sigma}{d\Omega}=\frac{const}{\Delta\Omega} \frac{N_{\gamma d \rightarrow pn}^{TRUE}}{N_\gamma}(1-BKG)
\end{equation}

where the factor (1-BKG) represents correction for the contribution of background events to the cross 
and the factor

\begin{equation}
\label{eff}
N_{\gamma d \rightarrow pn}^{TRUE} = \frac{N_{\gamma d \rightarrow pn}^{MEAS}}{\epsilon_{CLAS}}
\end{equation}

involves the knowledge of $\epsilon_{CLAS}$ representing the overall detector acceptance which 
reflects the geometrical inefficency in the detector setup and eventual damages in the apparatus.
For instance, the six superconducting coils of the CLAS toroidal magnet
are not covered by any active device so they cast a ``shadow'' in phase space which eats up 
events from the final state. On the other end, detector damages are connected to any kind of dead channels;
the most prominent contribution to this form of inefficency comes from the CLAS drift chambers which, 
after few years of running show several ``holes'' due to broken wires. 
The same can be said for the Time Of Flight system. 

To account for these effects one needs to simulate enough events with a single proton in the 
final state and to evaluate how many of them survive after running through the whole
analisis chain. In our case we have chosen to generate $10^6$ events of the type 
$\gamma d \rightarrow p n$. This was enough to have a statistical error comaprable with the one
coming from other factors in \ref{expcrosssect}.
\par
The generation of the photodisintegration events has been done using only pure kinematics.
This means that the angular distribution of protons in the c.m. system is uniform in $\theta$ 
and  $\phi$ and the only distorsion in the laboratory system is introduced by the Lorentz boost.
The photon energy spectrum ranges from 0.63 to 2.99 GeV corresponding to an electron beam 
energy of 3.15 GeV.
\par
The kinematical generator output has been processed by the CLAS GEANT simulation tool
(GSIM) and by the GSIM Post Processor (GPP) which takes into account several
real world issues such as the finite resolution of the CLAS Drift Chambers and Time Of Flight
systems, and holes due to dead channles in both these two detector components.

The smearing factors have been determined looking at the experimental width of the missing mass distribution
for the neutron. [MORE...]
\par

The BOS file processed as described above contains the same information of a physics file coming 
from the data acquisition system, but it contains additional infomation for the generated events 
which is stored in specific BOS banks which keep track of the original generated event.
This informations allows counting which and how many orignal events are missing after the reconstruction,
according to the relation:

\begin{equation}
\epsilon_{CLAS} = \frac{N_{\gamma d \rightarrow pn}^{REC} } {N_{\gamma d \rightarrow pn}^{GEN} }
\label{epsilon}
\end{equation}

Since the reconstructred BOS files are quite large and may contain unnecessary information
for the physics analysis. So, it is convenient to create custom Ntuples, which are more easily 
handeled by standard analysis tools and by the customized software we have written.
To obtain the CLAS acceptance funcion a simple algorithm scans the Ntuple  containing both
the reconstructed and the generated infomation and counts each generated event trying to match it
with the corresponding reconstruced event (i.e. proton).

For every kind of event corresponding the counter is incremented in each bin of $\theta,E_\gamma,\phi$.
Bins of 100 MeV in $E_\gamma$, $10^o$ in $\theta_{LAB}$, and $60^o$ (i.e., the six CLAS sectors) 
in $\phi$ were used. The code takes also into account the energy loss of the protons in crossing the 
the liquid deuterium target. 

Fiducial cuts were implemented to discard events that lie too close to the CLAS torus coils. 
which suffer to most from multiple scattering. To do so, a simple $\phi(\theta)$ 
function was used that produces a straight line cut in along each sector's side (fig ACCCUT).
....
\par
\par
Another source of inefficency is related to the signal to noise ratio.
This is intrinsic in any physical process, since always exists some some background contributions
from channels that can spoil the final state one is intesested in.
In our case the contribution to the missing mass spectrum are the following

\begin{itemize}
\item{ deuteron photodisintegration}
\item{ $\pi$ production on deutrium }
\item{ quasi-deuteron processes in the target windows}
\item{accidental coincidences between untagged high energy photons
and protons from either $\pi$ production processes or protons from photon interaction
in the target windows}
\item{accidental coincidences between untagged photons in the regular tagging range and protons from
pion production processes. The untagged photons are caused by the inefficency of the 
tagger spectrometer counters (around 3\%)}
\item{protons coming from a two step process in the deuterium target, specifically 
$\gamma d \rightarrow \pi^+ n n$ followed by $\pi^+ d \rightarrow p p$. Especially in backward
directions the combination of these processes can result in higher energy protons than the ones
coming from the deuteron break up} 
\end{itemize}

So, to take into account contamination from unwanted channels the background contribution
under the missing mass peak has to be evaluated. This can be done basically in two ways: 
a) from experimental data, b) from simulations.

In our case, an estimation of the signal with respect to the backgorund 
as a function of the proton scattering angle $\theta_{CM}$ is shown in figure 
\ref{background}, from which is clear that the statistics is not enough to have a 
complete background subtraction for all photon energies.

\begin{figure}[htb]
 \begin{center}
 \leavevmode
 \epsfig{file=background.eps,width=10cm}
 \caption{ }
 \label{fig:background}
 \end{center}
\end{figure}

From fig \ref{background} it is reasonable to assume that the background angular 
distribution does not vary with the photon energy. 
To estimate the background contributions to the missing mass spectrum for the neutron 
for each bin in $E_\gamma$ and $\theta$ one 
needs to simulate enough events over the whole photon energy range.
This is practically unfeasible because takes to much computing time and disk space.
For this reason, to check the above assumption it was decided
to simulate background events from the reaction $\gamma C \rightarrow X$ only for three 
specific photon energy bins, 0.6-0.7, 1.4-1.5, and 2.7-2.8 GeV.


means to take into account those events coming from the interaction with the 
carbon atoms contained in the mylar target walls.
 
The event generator program (GENBOS) extracts events taking into account known cross 
section from tabulated data.

\par
Background events have been generated also on deuteron, but in this case they are not 
contaminating directly the missing mass peak for the photodisintegration process which
has a threshold energy of 2.2 MeV much lower than any other competing process.


The BOS files containing all the events have been summed, with appropriate weights.


Then all the bins are divided according to the relation


\be
\frac{ N_{\gamma d \rightarrow p n}^{GEN} } {N_{\gamma d \rightarrow p n }^{REC} + w_d(E_\gamma,\theta,\phi) N_{\gamma d \rightarrow p X}^{REC} + w_C (E_\gamma,\theta,\phi) N_{\gamma C \rightarrow p X}^{REC} } 
\label{accfun}
\ee

having considered as 1 the weight for the deutron break-up events 

\begin{equation}
w_A(E_\gamma,\theta,\phi) = \frac{1}{E_\gamma} \frac{N_{\gamma d \rightarrow p n}^{GEN}  } {N_{\gamma A \rightarrow p X }^{GEN}  } \frac{ \frac{\Delta\sigma}{\Delta\theta\Delta\phi \Delta E_\gamma}\left(\gamma A \rightarrow p X \right) }{\frac{\Delta\sigma}{\Delta\theta\Delta\phi\Delta E_\gamma}\left(\gamma d \rightarrow p n \right)}
\end{equation}

The C program for the acceptance calculation outputs a text file with the acceptance funcion values 
foreach bin in $(E_\gamma,\theta,\phi$) and an HBOOK file containing a monitor ntuple and histograms.

The acceptance function si showed in fig. ACCFUN as a function of $\theta_{LAB}$ and integrated over 
the photon energy spectrum.

 

